Valid Explanations for Learning to Rank Models

Learning-to-rank (LTR) is a class of supervised learning techniques that apply to ranking problems dealing with a large number of features. The popularity and widespread application of LTR models in prioritizing information in a variety of domains makes their scrutability vital in today's landscape of fair and transparent learning systems. However, limited work exists that deals with interpreting the decisions of learning systems that output rankings. In this paper we propose a model agnostic local explanation method that seeks to identify a small subset of input features as explanation to a ranking decision. We introduce new notions of validity and completeness of explanations specifically for rankings, based on the presence or absence of selected features, as a way of measuring goodness. We devise a novel optimization problem to maximize validity directly and propose greedy algorithms as solutions. In extensive quantitative experiments we show that our approach outperforms other model agnostic explanation approaches across pointwise, pairwise and listwise LTR models in validity while not compromising on completeness.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios

==> old/old-expt-completeness.tex <==

% The optimal explanation for maximizing completeness is to choose all instances is the entire feature space $\f = \f'$. 
An explanation with high validity might not exhibit high completeness.
While a small number of features may prove to be sufficient for good valid explanations, the same does not hold for completeness. 
The inherent feature correlations found in real world data mean that simply removing a seemingly important feature may not affect completeness if there exists another feature correlated to it that the LTR model also focuses on. 

However large feature subsets tend be unwieldy as explanations for humans. Hence values of completeness close to $1$ is the exception rather than the norm with small explanation sizes. Note that completeness values close to 0 indicate that approximately half the concordant pairs from $\pi$ have been made discordant in $\pi'$ by removing a relatively small set of features.


From Table~\ref{tab:mq2008}, we first observe that removing a small random set of features has relatively low impact on the rank order of $\pi'$ (especially for the pairwise model where completeness is $-0.634$). 
Removing 5 important features attributed by \shap{} results in significant gains ($-0.071$ as compared to $-0.634$). 
%\todo{Megha: isn't it a good thing ? If teh correlation comes out to be close to 0 ,w e should be happy. It says once you remove teh valid features, tehr resulting ranking is no more correlated with the true ranking, of curse a negative correlation is even better nut i think a 0 correlation is still good enough and says that you definitely need the features that you removed}


%Hence we observe performance when selecting a small feature subset that has a relatively high impact on completeness. 
%Note that a value close to 0 does not mean the method is ineffective. It instead implies that exactly half of the concordant pairs in $\pi$ are discordant in $\pi'$ by just removing $k$ features.

%Now we examine the completeness metric for completeness optimized approaches. We see that at least one of our variants outperforms both \textsc{SHAP} approaches for all models. The choice of variant is highly dependent on the type of model. c. \greedy tends to be the best choice for the pointwise and listwise model whereas c. \greedycov is best for pairwise models. We find empirically that using our selected threshold when optimizing for completeness is a suboptimal choice. In our experiments we use the same threshold computation method for validity and completeness optimization. We leave threshold tuning specifically for completeness to future work.

Our experiments indicate that the there is no clear winner for completeness. Although our approach specifically optimizes for validity with the added constraint of a small explanation size, we are still competitive in terms of completeness and even better in some cases. 
\greedy is able to uncover more complete explanations especially for the pairwise model. For pointwise models our greedy approaches outperform \shap{} although only by a small margin. 
For listwise models in our experiments, the dataset influences whether \shap{} or our approach is a better choice. 

Out of our approaches, \greedy tends to be more complete except for the pointwise model in \mq{} where it is second best overall. 
\greedy does not take redundancy of feature contributions into account since coverage of pairs in not modelled here. 
Hence it is more likely to select correlated features as compared to \greedycov or \greedycovep reducing its informativeness and validity.

\mpara{Anecdotal example.} For example, \greedy selects the following features as an explanation for query $823$ (from \mslr{}) and the pairwise ranker: BM25 score of the body, LM score of the body, covered query term ratio of the title, sum of stream length normalized term frequency for the URL and covered query term number for the title whereas \greedycovep selects LM of the whole doc, sum of stream length normalized term frequency for the URL and covered query term number for the body. The LM and BM25 score of the body are highly correlated but only the LM score is selected by \greedycovep. This results in a completeness score of $-0.1$ for \greedy and $-0.6$ for \greedycovep.

%Also we see that \greedy has the best completeness for the pointwise model. 

A subtler takeaway here is that maximizing validity does not always mean minimizing completeness. 
This points to the presence of features that are both valid and complete. 
Finding an explanation that is both valid and complete is a challenging problem due to the dual nature of the objectives (one minimizes rank correlation while the other maximizes it) and we leave this to future work.

%Finally we observe Table~\ref{tab:mslrfull}. Since \textsc{MSLR} has 3 times as many features as \textsc{MQ2008}, we look at both $k=5$ and $k=10$. Most of the same trends hold here with v. \greedycovep being the best approach for the validity metrics and surprisingly for completeness for the pointwise model when $k=5$. For listwise approaches, all our completeness optimized variants are best performing in the completeness metric. 

%\todo{discuss that performance improves when going from 5 to 10 features}





==> preliminaries.tex <==





%\mpara{Basics. }
Learning to Rank (LTR) refers to training a machine learning model for a ranking task, for example, in document retrieval, recommender systems etc. 
% Learning to rank (LTR) refers to a family of machine learning algorithms in building ranking models for ranking tasks primarily arising in information retrieval and recommender systems.
% The training data in LTR consists of lists of items with some partial order specified between items in each list. 
% This order is typically induced by giving a numerical or ordinal score or a binary judgment (e.g. "relevant" or "not relevant") for each item. 
% The ranking model's purpose is to produce a permutation of items in new, unseen lists in a way which is "similar" to rankings in the training data in some sense.
We focus on document retrieval/ranking task, where given a query $\q$ we are interested in a ranking of documents that is most relevant to $\q$.
Consider a document collection $\mathcal{D}$ where we denote each document as $\doc \in \coll{}$. 
Document-query pairs are represented by feature vectors, that is, for a given query $\q$, its associated document $\doc$ can be represented by a feature vector $\x \,=\,\omega(\doc, \q) \in \mathbb{R}^{n} $, where $\omega$ is some feature extractor.
Typical features used in LTR include the frequencies of the query terms in the document, the BM25 and PageRank scores. With respect to training, LTR methods are trained either in a pointwise, pairwise, or listwise manner~\cite{liu2009learning}. In a pointwise approach, the LTR problem is cast into a regression problem where the goal is to predict a ranking score for a query-document pair. The pairwise approach, on the other hand, trains a binary classifier model that classifies the document preference pair as concordant or discordant. In particular, the model predicts a probability the input pair is concordant. We utilize these output probabilities for the input ordered document pairs as scores in our approach.
Finally, listwise approaches  directly optimize the value of ranking evaluation measures, like MAP, NDCG, averaged over all queries in the training data. 

%\todo{Megha: the definition of these notations is anywways repeated in the next sections, so I comment them out here}
% In the rest of the paper we use the following notations unless otherwise stated. We denote a LTR function $r(\f) \to \pi$ that produces a ranking $\pi$ of documents $\doc \in \coll$ given a query $\q$ over a feature set $\f$. If for document query pairs $\x_i$ and $\x_j$, the scores are such that $\Phi(\x_i) > \Phi(\x_j)$, then the document corresponding to $\x_i$ is ranked higher than the one corresponding to $\x_j$.
% Irrespective of the choice of the learning method, a scoring function is learnt that ranks documents in terms of descending value of the score $\Phi(\x)$.



% In a pointwise approach, it is assumed that each query-document pair in the training data has a numerical or ordinal score. Then the LTR problem can be approximated by a regression model — given a single query-document pair, predict its score.
%\todo{is the notation $d_i > d_j$ correct? }
% In a pairwise approach, the LTR problem is approximated by a classification problem, i.e., learning a binary classifier that classifies a preference
% pair $d_i > d_j$ as concordant or discordant. The goal in such methods is to minimize the average number of inversions/ discordance with the target ranking.
% This is typically hard because most evaluation measures are not continuous functions w.r.t to the parameters of the ranking model. Consequently, continuous approximations or bounds on evaluation measures have been proposed\cite{taylor2008softrank}.




% The result list of documents for $\q$ is denoted as $R(\q) = \pi$ and is sorted by a specified $f$. 






==> related-work.tex <==
\section{Related Work}
\label{sec:related-work}





==> related_work_expanded.tex <==
\section{Related Work }
\label{sec:related-work}

% Interpretability in machine learning has been studied extensively in classical machine learning. However, the success of neural networks (NN) and other expressive yet complex ML models have only intensified the discussion.

% Most of the success of NN models arise from the fact that they are powerful function approximators and have succeeded in learning complex non-linear hidden representations from raw input high-dimensional representations. On one hand they have largely improved performance, but on the other they tend to be opaque and less interpretable. Consequently, interpretability of these complex models has been studied in various other domains to better understand decisions made by the network -- image classification and captioning~\cite{captioningxu2015showattention,dabkowski2017real,imageclasssimonyan2013deep}, sequence to sequence modeling~\cite{seqalvarez2017causal,nlp2015visualizing}, recommender systems~\cite{interpretrecsysChang:2016} etc. 

% Post-hoc methods for interpretability can be categorized into two broad classes: \emph{model introspective} and \emph{model agnostic}. Model introspection refers to either interpretability by design or access to all the model parameters. In interpretability by design, more inherently ``interpretable'' models such as decision trees, rules~\cite{rulesletham2015interpretable}, additive models~\cite{caruana2015intelligibletrees} and attention-based networks~\cite{captioningxu2015showattention} are utilized. Instead of supporting models that are functionally black-boxes, such as an arbitrary neural network or random forests with thousands of trees, these approaches use models in which there is the possibility of meaningfully inspecting model components directly, e.g. a path in a decision tree, a single rule, or the weight of a specific feature in a linear model. 
Learning to Rank refers to training a machine learning model to predict a ranking, for example, for documents in a document retrieval task, or for items in recommender systems etc. 
% Learning to rank (LTR) refers to a family of machine learning algorithms in building ranking models for ranking tasks primarily arising in information retrieval and recommender systems.
% The training data in LTR consists of lists of items with some partial order specified between items in each list. 
% This order is typically induced by giving a numerical or ordinal score or a binary judgment (e.g. "relevant" or "not relevant") for each item. 
% The ranking model's purpose is to produce a permutation of items in new, unseen lists in a way which is "similar" to rankings in the training data in some sense.
In this work, we focus on document retrieval/ranking task, where given a query $\q$ the trained LTR model outputs a ranking of documents that is most relevant to $\q$. We are then interested in explaining the decision of the LTR model for a given output ranking with respect to the query $\q$. Interpretability approaches can be broadly grouped into two main classes:\textit{model-agnostic} and \textit{model-introspective} approaches.
% Consider a document collection $\mathcal{D}$ where we denote each document as $\doc \in \coll{}$. 
% Document-query pairs are represented by feature vectors, that is, for a given query $\q$, its associated document $\doc$ can be represented by a feature vector $\x \,=\,\omega(\doc, \q) \in \mathbb{R}^{n} $, where $\omega$ is some feature extractor.


Model agnostic methods formulate simple proxy models of full neural networks usually by learning a locally faithful approximation around the prediction, for example through linear models or sets of rules, representing sufficient conditions on the prediction \cite{rulesletham2015interpretable}. Model agnostic approaches for interpretability in rankings include \cite{singh2018posthoc} which constructed surrogate models to imitate decisions of black-box LTR models. Other works~\cite{Singhexs2019,Verma2019} adapt an existing local linear explanation model, LIME\cite{ribeiro2016should} to the problem of explaining document relevance with respect to a query. Both approaches deliver term based explanations for pointwise neural networks operating on raw text. We, on the other hand, focus on explaining LTR models with more understandable input features like frequencies of query terms in documents, the BM25 and PageRank scores. Moreover our approach is more general and can be applied additionally to pairwise and listwise approaches. Another line of work \cite{singh2020model} proposes an approach for locally explaining the ranked list output of pure text based neural rankers (that learn latent feature representations) via a set of intent terms. Our problem setting however is the more commonly prevailing setting in LTR where we have a known set of input features such as TF-IDF scores, page rank, etc. from which to choose an explanation.  A similar problem setting as ours can be found in \cite{ter2018faithfully} but it assumes access to original training data of the model which is not the case in our work.
% the approach is reliant on having a training set of rankings on which to learn an explainer. Our approach on the other hand does not require access to training data which is often unavailable in a truly model agnostic setting.
Model introspective methods identify important aspects of the computation, for example, through feature gradients\cite{zeiler2014visualizing}, backpropagation of neurons’ contributions to the input features \cite{shrikumar2017learning} etc. A model introspective approach was proposed by \cite{Fernando:2019:SIN:3331184.3331312} to interpret the relevance score of a single query document pair. 

In this work, we operate in the \textbf{model agnostic} regime where we do not assume any access to the ranking model's parameters. As already discussed none of the existing works can be directly applied to our problem setting. We, therefore, adapt a popular interpretability technique \textit{Shapley Additive Explanations}, SHAP\cite{lundberg2017unified} for comparisons with our approach. SHAP draws inspirations game theoretic results and utilizes the framework of Shapley Values\cite{} to compute feature's importance or contribution to a prediction (for a specific input) as compared to its expected value. In Section~\ref{sec:compareSHAP} we describe the adaptation and limitations of SHAP for explaining ranking models.

% In certain cases where we have access to the model parameters but direct introspection is not possible, approaches such as~\cite{influencefunctionskoh2017understanding,sharchilev2018finding} (explanations through influential training examples) and~\cite{lundberg2017unified} (explanations through input attributions) are more useful. 
% \todo{somehow SHAP appears in model interospective section and then we use it as a baseline for out model agnostic approach. we need to change that somehow}

For other notions of interpretability and a more comprehensive description of the approaches we point the readers to~\cite{guidotti2018survey}. Other loosely related line of works is the explainability of recommender systems~\cite{Zhang:2019:EIW:3331184.3331649}. A key difference here is that the explanations for a product recommendation is dependent on the rich user interaction history. Other works~\cite{Balog:2019:TSE:3331184.3331211} detail how a transparent and scrutable model can be built directly instead of explaining it posthoc.

% Tangential but related to our line of work is the explainability of recommender systems. We point readers to~\cite{Zhang:2019:EIW:3331184.3331649} for an overview of the field. A key difference to ranking models is that explanations here focus on explaining why a product was recommended to a user who has a rich interaction history. Recent works such as~\cite{Balog:2019:TSE:3331184.3331211} detail how a transparent and scrutable model can be built directly instead of explaining it posthoc.





% Recent work in this space has tended to focus on classification and regression models~\cite{ribeiro2016should,ribeiro2018anchors} but not on ranking models.
% Firstly, these works do not focus on interpreting intents and secondly they are not model agnostic limiting their usability.

%Model agnostic approaches on the other hand extract post-hoc explanations by treating the original model as a black box either by learning from the output of the black box model, or perturbing the inputs, or both~\cite{ribeiro2016should,influencefunctionskoh2017understanding}. Model agnostic interpretability is of two types: local and global. \emph{Local interpretability} refers to the explanations used to describe a single decision of the model. There are also other notions of interpretability, and for a more comprehensive description of the approaches we point the readers to~\cite{lipton2016mythos}.

% There is a line of work in machine learning where model parameters are accessible to the post-hoc explanation engine, or model-intrusive interpretability, and arguably the quality of explanations are better~\cite{binder2016layer,bach2015pixel,montavon2017explaining}.


% remove this and put in a paragraph about neural nets for ranking
% In IR there has been little to no work on post-hoc model agnostic interpretability. With the widespread adoption of neural networks in particular for a variety of text ranking tasks, we believe that model agnostic interpretability is crucial. Early models like DSSM~\cite{mitra2017neural} learned representations of text good for ranking using only character trigrams. Match Pyramid~\cite{pang2016study} learns feature maps using convolutional neural nets on query-document interaction matrices. More recent models such as DUET~\cite{mitra2016dual} take both into account making them even harder to interpret. Additionally models such as PACRR~\cite{} take term sequence and term position into account and claim start of the art results. While it has been empirically shown that these approaches outperform simpler and easier to understand IR baselines like BM25, it is difficult to answer the questions posed in the previous section regarding why a document is relevant or considered more relevant than another.


%Recently~\cite{Singhexs:2019, Verma:2019:LLI:3331184.3331377} demonstrated how local document perturbations can be used to find terms influencing the relevance of a query-document pair given a black box pointwise ranker. Here the terms that influence the relevance score arise only due to interaction between the query model and the document model.


% \mpara{Interpretability for Rankings:} In information retrieval there has been limited work on interpreting rankings.
%\todo{please check this again: even our work suffers from the same limitation. I believe the difference form our work is that it is a perturbation based method~\cite{ter2018faithfully} estimated the feature importance of a document in a ranked list given a learned ranker. This becomes unwieldy if the number of features is large or uninterpretable itself. JS: i had a look at this paper. they also do things similar to us. they use perturbations but also train a NN to predict the explanation from the ranking. they train this model using explanations from their method for the train set queries. Using their method is quite slow since it considers all permutations. we my have to compare against this if we mention it. they tackle the exact same problem as us. The paper isn't peer reviewed so we can leave it out.} 
%\todo{ I changed the description, is it what it does ? \cite{singh2018posthoc} approximated an already trained learning to rank model by a decision tree proxy model which was trained using a subset of the original features and the actual output of the original model. }
%They approximated an LTR model by a decision tree proxy model which was trained using a subset of the original features and the actual output of the original model
% A model introspective approach was proposed by \cite{Fernando:2019:SIN:3331184.3331312} to interpret the relevance score of a single query document pair. Recently several model-agnostic approaches have also been proposed. \cite{singh2018posthoc} describes a study on interpretable global surrogate models for LTR. \cite{Singhexs2019,Verma2019} are local model agnostic approaches which propose using the popular LIME~\cite{ribeiro2016should} method designed for classifiers on the task of explaining the relevance between a single query and document. 
%While the results of~\cite{Singhexs2019} are anecdotal, \cite{Verma:2019:LLI:3331184.3331377} evaluate how close complex ranking models are to the topic description as provided by TREC. 
%  In this work, we tackle the problem of listwise ranking. Closest to our work in terms of problem scope are~\cite{singh2020model,ter2018faithfully}.


\todo{We can potentially leave out \cite{ter2018faithfully} since it is not peer reviewed}
 



%\todo{please check if this holds for thsi work. This is different from our objective which is to accurately determine the intent terms that drive the ranking output of the model -- not just a single document and not how close it is to the intended intent for a given query. }


%they demonstrate anecdotally how document perturbations can be used to create local models to explain the relevance of a single query and document pair. 

%\todo{ I think the following part does not apply to the current workIn terms of approach we utilize similar perturbation techniques as the aforementioned works but only to identify a set of candidates. Instead of training a local classification or regression model, we optimize for ranking preferences directly for better intent determination.}



%\mpara{Feature Selection:} Feature Selection \cite{li2017feature} is a dimensionality reduction technique which aims at choosing a small subset of the relevant features from the original features by removing irrelevant, redundant or noisy features. Feature Selection is a preprocessing step that has been proven to be effective and efficient in preparing data (especially high-dimensional data) for various data mining and machine learning problems. \cite{geng2007feature} also showed the benefits of feature selection for ranking. 
%Our approach can also be seen as a \textit{filter} method for feature selection in which we select a small subset of features independent of the learning model satisfying the completeness and validity criteria for an explanation. 
%Our work is different from \cite{geng2007feature} not only in the optimization objectives but also due to the fact that our approach is used for explaining an already trained model, whereas \cite{geng2007feature} aims at finding the most important features prior to training a ranking model.

% Although the problem of explaining rankings is not a well studied problem, the problem of interpretability in various other domains such as image classification and captioning~\cite{captioningxu2015showattention,dabkowski2017real,imageclasssimonyan2013deep}, sequence to sequence modeling~\cite{seqalvarez2017causal,nlp2015visualizing}, recommender systems~\cite{interpretrecsysChang:2016} has received substantial attention. 


% Filter methods are feature select methods which are independent of learning model (and are therefore model agnostic) while selecting features are referred to as \emph{filter methods}. These can be further can be further categorized into two groups,
% namely,  feature  weighting  algorithms  and  subset
% search algorithms, based on whether they evaluate the importance of features individually or through feature subsets respectively. 

%Closest to our work is the recent work by Singh and Anand~\cite{singh2018posthoc} which tried to approximate an already trained learning to rank model by a subset of (the original features) interpretable features using secondary training data from the output of the original model. 
%Firstly, it does not focus on interpreting intents and secondly it is not model agnostic limiting its usability.

%\todo{Add SIGIR short papers. Zeons, LIRME,...} 

==> table.tex <==


\begin{table}[ht]

\begin{tabular}{lcccccccc}

\toprule

                             & \multicolumn{3}{c}{Validity $\uparrow$} &  & & \multicolumn{3}{c}{Completeness $\uparrow$} \\
                             & \texttt{Point }   & \texttt{Pair }    & \texttt{List }     &  & & \texttt{Point }     & \texttt{Pair }     & \texttt{List}      \\
\midrule
& \multicolumn{8}{c}{\textsc{MQ2008}} \\ \midrule
Random                       & 0.062   & 0.237   & 0.041    & & & -0.155    & -0.718   & -0.305    \\
\textsc{Shap-1}                        & 0.131   & 0.381   & 0.124    & & & 0.039     & -0.517   & -0.068    \\
\textsc{Shap-5}                        & 0.133   & 0.269   & 0.135    & & & 0.041     & -0.391   & \bf{-0.031}    \\
\midrule
\greedy               & 0.202   & 0.287   & 0.259    & & & 0.041     & \bf{-0.369}   & -0.091    \\
\greedycov         & 0.197   & 0.268   & 0.280   & &  & \bf{0.072}        & -0.371   & -0.096    \\
\greedycovep & \bf{0.299}      & \bf{0.616}   & \bf{0.361} &  &  & -0.013    & -0.623   & -0.162    \\

&  &  &  &  &  &  &  \\
\toprule
& \multicolumn{8}{c}{\textsc{MSLR}} \\ \midrule

Random & 0.002 & 0.009 & 0.000 & & & -0.172 & -0.634 & -0.303 \\
\textsc{Shap-1} & 0.006 & 0.050 & 0.023 & & & -0.007 & -0.071 & -0.052 \\
\textsc{Shap-5} & 0.009 & 0.048 & 0.001 & & & 0.000 & -0.067 & -0.051 \\ \midrule
\greedy & 0.007 & 0.060 & 0.045 & & & 0.001 & \bf{-0.057} & \bf{-0.034} \\
\greedycov & \bf{0.071} & 0.094 & \bf{0.081} & & & -0.025 & -0.130 & -0.070 \\
\greedycovep & 0.059 & \bf{0.110} & 0.074 & & & \bf{0.020} & -0.074 & -0.041 \\

\toprule
\end{tabular}

\caption{Results for the \textsc{MQ2008, MSLR} when k=5. All greedy approaches are statistically significantly better than the baselines for validity measures. \greedycovep is significantly better than its nearest competitor for validity.}
\label{tab:mq2008}
\end{table}


